Efficient Diffusion Policies for Offline Reinforcement Learning

Offline reinforcement learning (RL) aims to learn optimal policies from offline datasets, where the parameterization of policies is crucial but often overlooked. Recently, Diffsuion-QL significantly boosts the performance of offline RL by representing a policy with a diffusion model, whose success relies on a parametrized Markov Chain with hundreds of steps for sampling. However, Diffusion-QL suffers from two critical limitations. 1) It is computationally inefficient to forward and backward through the whole Markov chain during training. 2) It is incompatible with maximum likelihood-based RL algorithms (e.g., policy gradient methods) as the likelihood of diffusion models is intractable. Therefore, we propose efficient diffusion policy (EDP) to overcome these two challenges. EDP approximately constructs actions from corrupted ones at training to avoid running the sampling chain. We conduct extensive experiments on the D4RL benchmark. The results show that EDP can reduce the diffusion policy training time from 5 days to 5 hours on gym-locomotion tasks. Moreover, we show that EDP is compatible with various offline RL algorithms (TD3, CRR, and IQL) and achieves new state-of-the-art on D4RL by large margins over previous methods. Our code is available at https://github.com/sail-sg/edp.

==> tab/normal_ensemble.tex <==
\begin{table}[h]
\label{tab:reproduce}
\caption{Reproducing table}
\centering
\scriptsize
\newcolumntype{d}[1]{D{.}{.}{#1}}
\begin{tabular}{cS[table-format=3.2]S[table-format=3.2]S[table-format=3.2]} %{cccc} %{S[table-format=3.2]}
\toprule
Dataset                      & \multicolumn{1}{c}{DQL} & \multicolumn{1}{c}{DQL (Jax)} & \multicolumn{1}{c}{GDP}   \\
\midrule
halfcheetah-medium-v2        & 51.5        & 52.3               & 52.8  \\
hopper-medium-v2             & 96.6        & 95.3               & 98.6  \\
walker2d-medium-v2           & 87.3        & 86.9               & 89.6  \\
halfcheetah-medium-replay-v2 & 48.3        & 50.3               & 50.4  \\
hopper-medium-replay-v2      & 102.0       & 101.8              & 102.7 \\
walker2d-medium-replay-v2    & 98.0        & 96.3               & 97.7  \\
halfcheetah-medium-expert-v2 & 97.2        & 97.3               & 97.1  \\
hopper-medium-expert-v2      & 112.3       & 113.1              & 112.0 \\
walker2d-medium-expert-v2    & 111.2       & 111.5              & 112.0 \\
\rowcolor{shadecolor} gym-locomotion-v2 (avg)      & 89.4        & 89.4               & 90.3  \\
\bottomrule
\end{tabular}
\end{table}

==> tax/04_method_backup.tex <==
\section{Efficient Diffusion Policies}

In this section, we develop our efficient diffusion policies. First,  we formalize an RL policy with a diffusion model and explain why it is inefficient in the context of offline RL. Then, we detail our novel Reinforcement-Guided Diffusion Policy that makes policy evaluation and improvement much more efficient. Third, We show that our design is actually general and can be combined with arbitrary offline RL algorithms. In the end, we discuss several methods to sample from the diffusion policy during evaluation. 


\subsection{Diffusion Policy}

Following~\cite{wang2022diffusion}, we use the reverse process of a conditional diffusion model as a parametric policy: 
\begin{equation}
\label{eq:diff_policy}
    \pi_\theta(\vv{a}|\vv{s}) = p_\theta(\vv{a}^{0:K}|\vv{s}) = p(\vv{a}^K) \prod_{k=1}^K p_\theta(\vv{a}^{k-1}|\vv{a}^k, \vv{s}),
\end{equation}
where $\vv{a}^K \sim \mathcal{N}(\vv{0}, \vv{I})$. We choose to parameterize $\pi_\theta$ based on Denoising Diffusion Probabilistic Models (DDPM)~\cite{ho2020denoising}, which sets $\vv{\Sigma}_\theta(\vv{a}^k, k; \vv{s}) = \sigma_k^2 \vv{I}$ to fixed time-dependent constants, and constructs the mean $\vv{\mu}_\theta$ from a noise prediction model as: $\vv{\mu}_\theta(\vv{a}^k, k; \vv{s}) = \frac{1}{\sqrt{\alpha^k}} \left(\vv{a}^k - \frac{\beta^k}{\sqrt{1-\bar{\alpha}^k}} \vv{\epsilon}_\theta(\vv{a}^t, k; \vv{s}) \right)$,\tianyu{Add formulas of $\alpha^{k}=1-\beta^{k}$ and $\bar{\alpha}^k=\prod_{s=1}^{k}{\alpha}^s$; Check the use of $k$ and $t$} where $\vv{\epsilon}_\theta$ is parameterized with a neural network. Plugging in the conditional Gaussian distributions, the ELBO in Sec.~\ref{sec:pre_diffusion} can be simplified to the following training objective $L_{\text{diff}}(\theta)$: 
\begin{equation}
    \mathbb{E}_{k,\vv{\epsilon}, (\vv{a}^0, \vv{s})} 
    \left[ \left\| \vv{\epsilon} - \vv{\epsilon}_\theta \left(\sqrt{\bar{\alpha}^k} \vv{a}^0 + \sqrt{1-\bar{\alpha}^k} \vv{\epsilon}, k; \vv{s}\right) \right\|^2
    \right],
\end{equation}
where $k \in 1:K$\tianyu{define what is $1:K$. Besides, the expectation over $k$ should be weighted} is the diffusion steps from clean action to pure noise, $\vv{\epsilon} \in \mathcal{N}(\vv{0}, \vv{I})$, $(\vv{a}^0, \vv{s}) \in \mathcal{D}$ are state-action pairs drawn from the offline dataset. Given a dataset, we can easily and efficiently train a diffusion policy in a behavior-cloning manner as we only need to forward and backward through the network once each iteration. As shown in Diffusion-QL~\cite{wang2022diffusion}, diffusion policies can greatly boost the preformance when trained with TD3-based Q learning. However, it still faces two main drawbacks that limit its real-world application: 1) It is inefficient in sampling and training; 2) It is not generalizable to other strong offline reinforcement learning algorithms.

% Despite its effectiveness, such a diffusion policy is \textit{inefficient in sampling and training}, especially when it is combined with a reinforcement learning algorithm. 



% \subsection{Reinforcement Guided Diffusion Policy}
\subsection{Limitations of Diffusion Policy}
\paragraph{Sampling inefficiency} To sample action from a diffusion policy, one needs to draw samples from $K$ different Gaussian distributions sequentially, as illustrated in Eqn.~\eqref{eq:reverse_diff}-\eqref{eq:diff_policy}. With the reparametrization trick, the sampling process can be reformulated as 
% \textit{i.e.}, repeating the following for $K$ times: 
\begin{equation}
\label{eq:ddpm_sampling}
    \vv{a}^{k-1} = \frac{1}{\sqrt{\alpha^k}} \left(\vv{a}^k - \frac{\beta^k}{\sqrt{1-\bar{\alpha}^k}} \vv{\epsilon}_\theta(\vv{a}^t, k; \vv{s}) \right) + \sqrt{\beta^{k}} \vv{\epsilon}, 
\end{equation}
where $\vv{\epsilon} \sim \mathcal{N}(\vv{0}, \vv{I})$, $k = K,\dots,1$\tianyu{this is not standard. Better be `$k$ is the reverse timestep from $K$ to $0$'}. This requires us to forward the neural network $\vv{\epsilon}_\theta$ for $K$ times, which is in efficient when $K$ is large, \textit{e.g.}, 1000. 

% Fortunately, with the reparametrization trick, the above sampling process is differentiable, which makes training diffusion models with Q-learning tractable.

\paragraph{Training Inefficiency} We consider a typical Q-learning actor-critic framework for continuous control, which iterates between policy evaluation and policy improvement. Policy evaluation learns a Q network by minimizing the following TD error $L_\text{TD}(\phi)$:
\begin{equation}
\label{eq:td_error}
    \mathbb{E}_{(\vv{s},\vv{a},\vv{s}^\prime)\sim\mathcal{D}} \left[\left(r(\vv{s},\vv{a}) + \gamma Q_{\hat{\phi}}(\vv{s}^\prime, \vv{a}^\prime) - Q_\phi(\vv{s}, \vv{a})\right)^2  \right],
\end{equation}
where the next action $\vv{a}^\prime \sim \pi_\theta(\cdot|\vv{s}^\prime)$. The policy network is optimized to maximize the expected Q values : 
\begin{equation}
\label{eq:max_q}
    \max_\theta 
    \mathbb{E}_{\vv{s}\sim \mathcal{D}, \vv{a}\sim \pi_\theta(\vv{a} | \vv{s})}
    \left[Q_\phi(\vv{s}, \vv{a})\right].
\end{equation}

The training inefficiency comes from two parts when a diffusion policy is used in the above algorithm. 
First, calculating $L_\text{TD}(\phi)$ (Eqn.~\eqref{eq:td_error}) requires drawing the next action from it, which suffers sampling inefficiency. Second, to optimize the policy network with Eqn.~\eqref{eq:max_q}, an action must be drawn from the policy, then calculate the loss function and backpropagate through the sampling process. Unlike a normal policy network where we only need to forward and backward through it once, we now have to do it $K$ times, which is unaffordably expensive when $K$ is large or the network is heavy. 

\paragraph{Incompatibility} Moreover, with diffusion models, it is preventably complicated to obtain the log-likelihood of samples~\cite{put references}. However, most actor-critic RL algorithms require to calculate of the log-likelihood of actions $\log \pi_\theta(\vv{a} | \vv{s})$, so that they can optimize the network to maximize it. 

Next, we develop our Reinforcement Guided Diffusion Policy that is efficient to train and compatible with most RL algorithms. 

\subsection{Reinforcement Guided Diffusion Policy} 
\textcolor{orange}{how about `generalized diffusion policy`}

As discussed above, parametrizing policy with diffusion models but optimizing it as usual in RL is inefficient. In this paper, we propose to view the offline RL problem from the perspective of generative modeling and use reinforcement as guidance. More specifically, unlike traditional generative modeling in computer vision, where the training data are usually perfect, offline RL datasets often contain suboptimal state-action pairs. Therefore, it is important that we can learn Q values with RL methods to measure the quality of state-action pairs. Then the question becomes how we can efficiently use the learned Q values to guide diffusion policy training. 

We propose the Reinforcement Guided Diffusion Policy (RGDP) to avoid sampling and backpropagating through the reverse diffusion process. Let's revisit the forward diffusion process in Eqn.~\ref{eq:forward_diff}. A notable property of it is that the distribution of noisy action $\vv{a}^k$ at any step $k$ can be written in closed form: $q(\vv{a}^{k} | \vv{a}^0) = \mathcal{N}(\vv{a}^k; \sqrt{\bar{\alpha}^k} \vv{a}^0, (1-\bar{\alpha}^k) \vv{I})$, where $\alpha^k \triangleq 1 - \beta^k$ and $\bar{\alpha}^k \triangleq \prod_{s=1}^k \alpha^k$\tianyu{these definitions should be moved forward}. Using the reparametrization trick, we are able to connect $\vv{a}^0$ and $\epsilon$ with:
\begin{equation}
\label{eq:eps_to_at}
    \vv{a}^k = \sqrt{\bar{\alpha}^k} \vv{a}^0 + \sqrt{1-\bar{\alpha}^k}\vv{\epsilon}, \quad \vv{\epsilon} \sim \mathcal{N}(\vv{0}, \vv{I}).
\end{equation}
Recall that our diffusion policy is parameterized to predict $\vv{\epsilon}$ with $\vv{\epsilon}_\theta(\vv{a}^k, k; \vv{s})$. By relacing $\vv{\epsilon}$ with $\vv{\epsilon}_\theta(\vv{a}^k, k; \vv{s})$ and rearranging Eqn.~\eqref{eq:eps_to_at}, we obtain the approximiated action by:
\begin{equation}
\label{eq:eps_to_astart}
    \hat{\vv{a}}^0 = \frac{1}{\sqrt{\bar{\alpha}^k}} \vv{a}^k - 
    \frac{\sqrt{1-\bar{\alpha}^k}}{\sqrt{\bar{\alpha}^k}} \vv{\epsilon}_\theta(\vv{a}^k, k; \vv{s}). 
\end{equation}
Now, instead of running the reverse diffusion process to sample an action $\vv{a}^0$, we can cheaply construct $\hat{\vv{a}}^0$ from a start-action pair $(\vv{s}, \vv{a})$ with only once network forward using the above equation. Accordingly, the policy improvement objective is modified as follows:
\begin{equation}
\label{eq:max_q_pred}
    L_\pi (\theta) = - \mathbb{E}_{\vv{s}\sim \mathcal{D}, \hat{\vv{a}}^0} \left[ Q_\phi(\vv{s}, \hat{\vv{a}}^0)\right].
\end{equation}
In this way, the training efficiency for policy improvement can be substantially improved. To improve the efficiency of policy evaluation, we propose to replace the DDPM sampling in Eqn.~\eqref{eq:ddpm_sampling} with DPM-Solver~\cite{lu2022dpm}, which is an ODE-based sampler. DPM-Solver is able to reduce the sampling steps from 1000 to 15, thus further accelerating the training of diffusion policies. The overall algorithm for our Reinforcement Guided Diffusion Policy learning is given in Alg.~\ref{alg:rgdp}.

\begin{algorithm}[tb]
   \caption{Reinforcement Guided Diffusion Policy}
   \label{alg:rgdp}
\begin{algorithmic}
   \STATE {\bfseries Input:} weight $\lambda$, dataset $\mathcal{D}$, $ \vv{\epsilon}_\theta(\vv{a}^k, k; \vv{s})$, $Q_\phi(\vv{s}, \vv{a})$
   \REPEAT
   \STATE Sample a batch of data: $\{(\vv{s}, \vv{a}, \vv{s}^\prime)\} \sim \mathcal{D}$ 
   \STATE Sample next action: $\vv{a}^\prime \sim \pi_\theta(\cdot | \vv{s})$ with DPM-Solver
   \STATE Update Q-network: $\phi \leftarrow \phi - \eta \nabla_\phi L_\text{TD} (\phi)$ 
   \STATE Calculate $\hat{\vv{a}}^0$ with Eqn.~\eqref{eq:eps_to_astart}
   \STATE Update policy: $\theta \leftarrow \theta - \eta \nabla_\theta (L_\text{diff} (\theta) + \lambda L_\pi (\theta))$
   \UNTIL{converged}
\end{algorithmic}
\end{algorithm}


\subsection{Generalization to Various RL algorithms}
There are mainly two types of approachs to realize the objective in Eqn.~\ref{eq:max_q} during policy improvement. 

\textit{Direct policy learning}: It maximizes Q values and directly backprogate the gradients from Q network to policy network, \textit{i.e.}, $\nabla_\theta L_\pi (\theta) = -\frac{\partial Q_\phi (\vv{s},\vv{a})}{\partial \vv{a}} \frac{\partial \vv{a}}{\partial \theta}$. This is only applicable to cases where $\frac{\partial \vv{a}}{\partial \theta}$ is tractable, \textit{e.g.}, when a deterministic policy $\vv{a} = \pi_\theta(\vv{s})$ is used or when the sampling process can be reparameterized. Sample algorithms belong to this catetory include TD3~\cite{TD3} and CQL~\cite{CQL}.  Therefore, one can easily verified that both the expensive DDPM sampling in Eqn.~\eqref{eq:ddpm_sampling} and our efficient approximation in Eqn.~\eqref{eq:eps_to_astart} can be used for direct policy learning. 

\textit{Indirect policy learning}: It tries to distill the knowledge from Q network into the policy network indirectly by performing weighted regression or weighted maximum likelihood:
\begin{equation}
\label{eq:indirect_policy}
    \mathbb{E}_{(\vv{s}, \vv{a}) \sim \mathcal{D}} \left[ w(Q_\phi(\vv{s},\vv{a})) \log \pi_\theta(\vv{a}|\vv{s}) \right],
\end{equation}
where $w(Q_\phi(\vv{s},\vv{a}))$ is a monotone increasing function that assigns a weight to each state-action pair in the dataset. This objective requires the log-likelihood of the policy is tractable and differentiable. AWR~\cite{AWR}, CRR~\cite{CRR} and IQL~\cite{IQL} fall into this category but each has a unique design in terms of the weighting function $w$. We propose the following two variants for realizing Eqn.~\ref{eq:indirect_policy}. 

First, following DDPM~\cite{ho2020denoising}, we have the following lower bound for $\log \pi_\theta(\vv{a}|\vv{s})$:\tianyu{the likelihood of using SDE solver (e.g., DDPM) and ODE solver (e.g., DPM-Solver) are different. Besides, there should be an extra term of KL divergence between priors}
\begin{equation}
    \mathbb{E}_{k,\vv{\epsilon}, (\vv{a}, \vv{s})} 
    \left[ \frac{(\beta^k)^2}{2(\sigma^k)^2 \alpha^k (1-\bar{\alpha}^k)} \left\| \vv{\epsilon} - \vv{\epsilon}_\theta \left(\vv{a}^k, k; \vv{s}\right) \right\|^2
    \right],
\end{equation}
where $\vv{a}^k = \sqrt{\bar{\alpha}^k} \vv{a} + \sqrt{1-\bar{\alpha}^k} \vv{\epsilon}$. Therefore, we ca have a lowerbound for the wegithed regression objective as below:
\begin{equation}
    \mathbb{E}_{k,\vv{\epsilon}, (\vv{a}, \vv{s})} 
    \left[ \frac{(\beta^k)^2 \cdot  w(Q_\phi(\vv{s}, \vv{a}))}{2(\sigma^k)^2 \alpha^k (1-\bar{\alpha}^k)} \left\| \vv{\epsilon} - \vv{\epsilon}_\theta \left(\vv{a}^k, k; \vv{s}\right) \right\|^2
    \right].
\end{equation}

Second, instead of directlying optimizing $\log \pi_\theta(\vv{a}|\vv{s})$, we propose to replace it with an approximated policy $\hat{\pi}_\theta(\vv{a} | \vv{s}) \triangleq \mathcal{N}(\hat{\vv{a}}^0, \vv{I})$, where $\hat{\vv{a}}^0$ is from Eqn.~\eqref{eq:eps_to_astart}. Then, we have the following objective for policy improvement:
\begin{equation}
    \mathbb{E}_{k,\vv{\epsilon}, (\vv{a}, \vv{s})} 
    \left[  w(Q_\phi(\vv{s}, \vv{a})) \left\| \vv{a} - \hat{\vv{a}}^0 \right\|^2
    \right].
\end{equation}
Emperically, we find these two choices perform similary but the latter one is easier to implement. So we will report results mainly based on the second realization. 

% $\max_\theta \mathbb{E}_{\vv{s}\sim \mathcal{D}}[Q_\phi (\vv{s}, \pi_\theta(\vv{s}))]$.


% \subsubsection{Energy-based Action Selection}
\subsection{Controlled Sampling from Diffusion Policies}
Traditionally, a continous policy is represented with a state-conditional Gaussian distribution. During eluvation time, researchers usually deteriminsticly use the distribution mean as action to reduce variance. However, with diffusion polices, we can only randomly drawn a sample from the underlying distribution without accessing to its statistics. As a result, the sampling process is nosiy and the evaluation is of high variance. To reduce evaluation variance, we propose \emph{Energy-based Action selection}. 


\paragraph{Sampling from $\pi^\tau_\theta(\vv{a}|\vv{s})$, $\tau > 1$}

\paragraph{Energy-based Guidance}

\paragraph{Energy-based Action selection}
Consider $p(\vv{a}|\vv{s}) \propto e^{Q(\vv{s},\vv{a})} \pi_\theta(\vv{a}|\vv{s})$, which is hard to sample from. We propose to first sample $N$ actions  from $\pi_\theta$ by using any samplers (\textit{i.e.}, DPM-Solver), then sample one of them with weights proportional to $ e^{Q(\vv{s},\vv{a})}$, as given by:
\begin{algorithm}[h]
   \caption{Energy-based Action Selection}
   \label{alg:energy_action}
\begin{algorithmic}
   \STATE {\bfseries Input:} number of actions: $N$, $\pi_\theta(\vv{a}|\vv{s})$, $Q_\phi(\vv{s}, \vv{a})$
   \STATE $\vv{a}_i \sim \pi_\theta(\vv{a}|\vv{s}) \quad i = 1, \dots, N$
   \STATE $\vv{a} = $ \texttt{categorical\_sample}($\{\vv{a}_i\}$, $\{e^{Q_\phi(\vv{s},\vv{a}_i)}\}$)
   \STATE {\bfseries  Output:} $\vv{a}$
\end{algorithmic}
\end{algorithm}

